Tuning Multigrid Methods with Robust Optimization

Local Fourier analysis is a useful tool for predicting and analyzing the performance of many efficient algorithms for the solution of discretized PDEs, such as multigrid and domain decomposition methods. The crucial aspect of local Fourier analysis is that it can be used to minimize an estimate of the spectral radius of a stationary iteration, or the condition number of a preconditioned system, in terms of a symbol representation of the algorithm. In practice, this is a "minimax" problem, minimizing with respect to solver parameters the appropriate measure of work, which involves maximizing over the Fourier frequency. Often, several algorithmic parameters may be determined by local Fourier analysis in order to obtain efficient algorithms. Analytical solutions to minimax problems are rarely possible beyond simple problems; the status quo in local Fourier analysis involves grid sampling, which is prohibitively expensive in high dimensions. In this paper, we propose and explore optimization algorithms to solve these problems efficiently. Several examples, with known and unknown analytical solutions, are presented to show the effectiveness of these approaches.

==> Makefile <==
# Makefile for 


#HEADER = Optimization_LFA
HEADER = rev1
PICS = images
BIB = LFA_Optimization
TEX = .
#TR = P9004-1017

TARGETS: $(HEADER).pdf

tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
pic_files = $(shell find $(PICS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
	)

%.pdf: %.tex $(tex_files) $(bib_files) $(pic_files)
	pdflatex -shell-escape $(HEADER)
	bibtex $(HEADER)
	pdflatex -shell-escape $(HEADER)	
	pdflatex -shell-escape $(HEADER)	
#	pdflatex -shell-escape $(TR)	

clean:
	find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
		\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
		\( -name '*.spl' -print \) -or \
		\( -name '*.bcf' -print \) -or \
		\( -name '*.out' -print \) -or \
		\( -name '*.out.ps' -print \) -or \
		\( -name '*.thm' -print \) -or \
		\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
		\( -name '*.log' -print \) -or \( -name '*.brf' -print \) -or \
		\( -name '*.toc' -print \) -or \( -name '*.toc.old' -print \) | xargs rm -f; \
	rm -f $(HEADER).dvi $(HEADER).log $(HEADER).ps $(HEADER).pdf $(HEADER).out \
		_region_* TAGS 

